LLM4DV: Using Large Language Models for Hardware Test Stimuli Generation

Hardware design verification (DV) is a process that checks the functional equivalence of a hardware design against its specifications, improving hardware reliability and robustness. A key task in the DV process is the test stimuli generation, which creates a set of conditions or inputs for testing. These test conditions are often complex and specific to the given hardware design, requiring substantial human engineering effort to optimize. We seek a solution of automated and efficient testing for arbitrary hardware designs that takes advantage of large language models (LLMs). LLMs have already shown promising results for improving hardware design automation, but remain under-explored for hardware DV. In this paper, we propose an open-source benchmarking framework named LLM4DV that efficiently orchestrates LLMs for automated hardware test stimuli generation. Our analysis evaluates six different LLMs involving six prompting improvements over eight hardware designs and provides insight for future work on LLMs development for efficient automated DV.

==> figures/config_comp.tex <==
\begin{figure}
\begin{tikzpicture}[thick,scale=0.95, every node/.style={scale=0.95}]
\pgfplotsset{every x tick label/.append style={font=\footnotesize}, compat=1.3,
table/search path={data/config_comp}}
\begin{axis}[
    height=80mm,
    width=\textwidth,
    xlabel={\footnotesize Message Count},
    ylabel={\footnotesize Coverage Rate},
    % ylabel style = {align=center},
    xmin=0, 
    % ymax = 32, ymin = 3.0517578125e-05,
    xtick={10, 20, 100, 500},
    % ymode=axis, 
    xmode=log,
    legend cell align={left},
    % log basis y={2},
    log ticks with fixed point,
    % scaled x ticks = false, 
    % scaled y ticks = false,
    % legend columns = 1,
    legend style={at={(0.04,0.95)},anchor=north west, draw=none, fill=none, font=\footnotesize},
    yticklabel={$\pgfmathprintnumber{\tick}\%$}
    ]
% claude-3-sonnet_1_I_a_i
\addplot[jcpurple, draw=jcpurple, mark=, line width=1.5pt, mark options={scale=0.7}] table
[x=Total Message, y=Coverage Rate, col sep=comma] {claude-3-sonnet_1_I_a_i.csv};
\addlegendentry{1 I a i}

% claude-3-sonnet_1_IV_a_iii
\addplot[jcred, draw=jcred, mark=, line width=1.5pt, mark options={scale=0.7}] table
[x=Total Message, y=Coverage Rate, col sep=comma] {claude-3-sonnet_1_IV_a_iii.csv};
\addlegendentry{1 IV a iii}

% claude-3-sonnet_2_II_a_iii
\addplot[jcgreen, draw=jcgreen, mark=, line width=1.5pt, mark options={scale=0.7}] table
[x=Total Message, y=Coverage Rate, col sep=comma] {claude-3-sonnet_2_II_a_iii.csv};
\addlegendentry{2 II a iii}

% claude-3-sonnet_2_II_b_i
\addplot[jcblue, draw=jcblue, mark=, line width=1.5pt, mark options={scale=0.7}] table
[x=Total Message, y=Coverage Rate, col sep=comma] {claude-3-sonnet_2_II_b_i.csv};
\addlegendentry{2 II b i}

% claude-3-sonnet_2_II_c_iii
\addplot[jcbrown, draw=jcbrown, mark=, line width=1.5pt, mark options={scale=0.7}] table
[x=Total Message, y=Coverage Rate, col sep=comma] {claude-3-sonnet_2_II_c_iii.csv};
\addlegendentry{2 II c iii}

% claude-3-sonnet_2_IV_a_iii
\addplot[black, draw=black, mark=, line width=1.5pt, mark options={scale=0.7}] table
[x=Total Message, y=Coverage Rate, col sep=comma] {claude-3-sonnet_2_IV_a_iii.csv};
\addlegendentry{2 IV a iii}

% claude-3-sonnet_3_II_b_iii
\addplot[jcyellow, draw=jcyellow, mark=, line width=1.5pt, mark options={scale=0.7}] table
[x=Total Message, y=Coverage Rate, col sep=comma] {claude-3-sonnet_3_II_b_iii.csv};
\addlegendentry{3 II b iii}

% claude-3-sonnet_3_IV_a_ii
\addplot[jcorange, draw=jcorange, mark=, line width=1.5pt, mark options={scale=0.7}] table
[x=Total Message, y=Coverage Rate, col sep=comma] {claude-3-sonnet_3_IV_a_ii.csv};
\addlegendentry{3 IV a ii}

\end{axis}
\end{tikzpicture}    
\caption{Experiments on the Ibex CPU module. Each line represents the trial reaching the maximum coverage on a configuration. The configurations in legends are illustrated in Figure~\ref{LLM4DV_detailed}.}
\label{fig:config_comp}
\end{figure}

==> figures/few_shot_comp.tex <==
\begin{tikzpicture}[thick,scale=0.85, every node/.style={scale=0.85}]
\pgfplotsset{every x tick label/.append style={font=\footnotesize}, compat=1.3,
table/search path={data/few_shot_comp}}
\begin{axis}[
    height=60mm,
    width=1.17\textwidth,
    xlabel={\footnotesize Message Count},
    ylabel={\footnotesize Coverage Rate},
    % ylabel style = {align=center},
    xmin=1, 
    % ymax = 32, ymin = 3.0517578125e-05,
    xtick={10, 20, 60, 100, 250, 500},
    % ymode=axis, 
    xmode=log,
    legend cell align={left},
    % log basis y={2},
    log ticks with fixed point,
    % scaled x ticks = false, 
    % scaled y ticks = false,
    legend columns = 2,
    legend style={at={(0.01,0.99)},anchor=north west, draw=none, fill=none, font=\scriptsize},
    yticklabel={$\pgfmathprintnumber{\tick}\%$}
    ]
% gpt3
\addplot[jcred, draw=jcred, mark=, line width=1.5pt, mark options={scale=0.7}, dashed] table
[x=Total Message, y=Coverage Rate, col sep=comma] {gpt-3_few_shot.csv};
\addlegendentry{GPT-3 Few Shot}

\addplot[jcred, draw=jcred, mark=, line width=1.5pt, mark options={scale=0.7}] table
[x=Total Message, y=Coverage Rate, col sep=comma] {gpt-3_no_few_shot.csv};
\addlegendentry{GPT-3 }

% claude
\addplot[jcgreen, draw=jcgreen, mark=, line width=1.5pt, mark options={scale=0.7}, dashed] table
[x=Total Message, y=Coverage Rate, col sep=comma] {claude_few_shot.csv};
\addlegendentry{Claude3 Few Shot}

\addplot[jcgreen, draw=jcgreen, mark=, line width=1.5pt, mark options={scale=0.7}] table
[x=Total Message, y=Coverage Rate, col sep=comma] {claude_no_few_shot.csv};
\addlegendentry{Claude3 }

% claude - 3.5
\addplot[jcbrown, draw=jcbrown, mark=, line width=1.5pt, mark options={scale=0.7}, dashed] table
[x=x, y=y, col sep=space] {cld35_few_shot_with_cot.dat};
\addlegendentry{Claude3.5 Few Shot}

\addplot[jcbrown, draw=jcbrown, mark=, line width=1.5pt, mark options={scale=0.7}] table
[x=x, y=y, col sep=space] {cld35_zero_shot.dat};
\addlegendentry{Claude3.5 }

% llama2
\addplot[jcblue, draw=jcblue, mark=, line width=1.5pt, mark options={scale=0.7}, dashed] table
[x=Total Message, y=Coverage Rate, col sep=comma] {llama2_few_shot.csv};
\addlegendentry{Llama2 Few Shot}

\addplot[jcblue, draw=jcblue, mark=, line width=1.5pt, mark options={scale=0.7}] table
[x=Total Message, y=Coverage Rate, col sep=comma] {llama2_no_few_shot.csv};
\addlegendentry{Llama2 }

% codellama
\addplot[jcorange, draw=jcorange, mark=, line width=1.5pt, mark options={scale=0.7}, dashed] table
[x=Total Message, y=Coverage Rate, col sep=comma] {codellama_few_shot.csv};
\addlegendentry{CodeLlama Few Shot}

\addplot[jcorange, draw=jcorange, mark=, line width=1.5pt, mark options={scale=0.7}] table
[x=Total Message, y=Coverage Rate, col sep=comma] {codellama_no_few_shot.csv};
\addlegendentry{CodeLlama }

% llama3
\addplot[jcpurple, draw=jcpurple, mark=, line width=1.5pt, mark options={scale=0.7}, dashed] table
[x=Total Message, y=Coverage Rate, col sep=comma] {llama3_few_shot.csv};
\addlegendentry{Llama3 Few Shot}

\addplot[jcpurple, draw=jcpurple, mark=, line width=1.5pt, mark options={scale=0.7}] table
[x=Total Message, y=Coverage Rate, col sep=comma] {llama3_no_few_shot.csv};
\addlegendentry{Llama3 }

\end{axis}
\end{tikzpicture}
\caption{Performance improvement due to few-shot prompting on the IBEX CPU.}
\label{few_shot_comp}

==> figures/naive_vs_improved.tex <==
\begin{tikzpicture}[thick,scale=0.85, every node/.style={scale=0.85}]
\pgfplotsset{every x tick label/.append style={font=\footnotesize}, compat=1.3,
table/search path={data/naive_vs_improved}}
\begin{axis}[
    height=60mm,
    width=1.17\textwidth,
    xlabel={\footnotesize Message Count},
    ylabel={\footnotesize Coverage Rate},
    % ylabel style = {align=center},
    xmin=1, 
    % ymax = 32, ymin = 3.0517578125e-05,
    % xtick={10, 20, 60, 100, 250, 500},
    % ymode=axis, 
    % xmode=log,
    legend cell align={left},
    % log basis y={2},
    log ticks with fixed point,
    % scaled x ticks = false, 
    % scaled y ticks = false,
    % legend columns = 1,
    legend style={at={(0.6,0.25)},anchor=north west, draw=none, fill=none, font=\footnotesize},
    yticklabel={$\pgfmathprintnumber{\tick}\%$}
    ]
% Naive
\addplot[jcred, draw=jcred, mark=, line width=1.5pt, mark options={scale=0.7}] table
[x=Total Message, y=Coverage Rate, col sep=comma] {claude-3-sonnet_1_I_a_i.csv};
\addlegendentry{Naive (Claude-3 1 I a i)}

\addplot[jcblue, draw=jcblue, mark=, line width=1.5pt, mark options={scale=0.7}] table
[x=Total Message, y=Coverage Rate, col sep=comma] {claude-3-sonnet_2_II_a_iii.csv};
\addlegendentry{Improved (Claude-3 2 II a iii)}

\addplot[mark=none, black, dashed, line width=1pt] coordinates {(240, 51.53061224489800) (295, 51.53061224489800)};
\addplot[mark=none, black, line width=1pt, <->] coordinates {(283, 51.53061224489800) (283, 66.83673469387760)};

\node[black] at (axis cs: 245, 58) {$\Delta$ = 15.3\%};

% \addplot[mark=none, black, ->, line width=1pt] coordinates {(240, 51.53061224489800) (283, 66.83673469387760)};

\end{axis}
\end{tikzpicture}    
\caption{Performance improvement due to the employment of the four generic prompting strategies on the IBEX CPU, using Claude 3 Sonnet.}
\label{naive_vs_improved}


==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

